Physical-Layer Security via Distributed Beamforming in the Presence of Adversaries with Unknown Locations

We study the problem of securely communicating a sequence of information bits with a client in the presence of multiple adversaries at unknown locations in the environment. We assume that the client and the adversaries are located in the far-field region, and all possible directions for each adversary can be expressed as a continuous interval of directions. In such a setting, we develop a periodic transmission strategy, i.e., a sequence of joint beamforming gain and artificial noise pairs, that prevents the adversaries from decreasing their uncertainty on the information sequence by eavesdropping on the transmission. We formulate a series of nonconvex semi-infinite optimization problems to synthesize the transmission strategy. We show that the semi-definite program (SDP) relaxations of these nonconvex problems are exact under an efficiently verifiable sufficient condition. We approximate the SDP relaxations, which are subject to infinitely many constraints, by randomly sampling a finite subset of the constraints and establish the probability with which optimal solutions to the obtained finite SDPs and the semi-infinite SDPs coincide. We demonstrate with numerical simulations that the proposed periodic strategy can ensure the security of communication in scenarios in which all stationary strategies fail to guarantee security.

==> figure.tex <==

\begin{figure}[t!]\centering
\scalebox{0.6}{
\begin{tikzpicture}
% the origin
\coordinate (O) at (0,0);
% the circle and the dot at the origin
\draw[fill=green,opacity=0.6] (O) node[circle,inner sep=1pt,fill] {} circle [radius=1cm] node[anchor=north,opacity=1] {};

\draw (O) node[circle,inner sep=1pt,fill] {} circle [radius=2cm];
% the ``\theta'' arc
\draw[dashed] 
  (-15:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (15:3.2) coordinate (slcoord)
  pic [angle radius=1.3cm,"$\delta$"] {angle = xcoord--O--slcoord};

  \draw[dashed] 
  (80:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (80:3.2) coordinate (slcoord);
  \draw[dashed] 
  (100:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (100:3.2) coordinate (slcoord);
  \draw[dashed] 
  (130:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (130:3.2) coordinate (slcoord);
  \draw[dashed] 
  (148:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (148:3.2) coordinate (slcoord);
  \draw[dashed] 
  (192:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (192:3.2) coordinate (slcoord);
  \draw[dashed] 
  (248:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (248:3.2) coordinate (slcoord);
  \draw[dashed] 
  (295:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (295:3.2) coordinate (slcoord);
  \draw[dashed] 
  (305:3.2) coordinate (xcoord) -- 
  node[midway,below] {} (O) -- 
  (305:3.2) coordinate (slcoord);

\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (-13:3cm)$) arc (-13:13:3cm) node [midway,right] {$I_0$};

\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (17:3cm)$) arc (17:78:3cm) node [midway,above] {$I_1$};
\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (102:3cm)$) arc (102:128:3cm) node [midway,above] {$I_2$};
\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (150:3cm)$) arc (150:190:3cm) node [midway,left] {$I_3$};
\draw[] (-2.5,-2) node [rotate=-45] {$\ldots$};
\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (250:3cm)$) arc (250:293:3cm) node [midway,below] {$I_{L-1}$};
\draw[|-|]
  % radius=3mm, initial=0, final=90
  %([shift={(0:3mm)}]c1) arc (0:90:3mm)
  ($(O) + (307:3cm)$) arc (307:343:3cm) node [midway,below, yshift=-5pt] {$I_L$};
 
  \draw[fill]
  ($(O) + (15:0.5cm)$) arc (15:-15:0.5cm); 
  
  \draw[fill=red,opacity=0.6]
  ($(O) + (15:2cm)$) arc (15:80:2cm)
  --
  ($(O) + (80:2.5cm)$) arc (80:15:2.5cm)
  -- cycle;
  \draw[fill=red,opacity=0.6]
  ($(O) + (100:2cm)$) arc (100:130:2cm)
  --
  ($(O) + (130:2.5cm)$) arc (130:100:2.5cm)
  -- cycle;
  \draw[fill=red,opacity=0.6]
  ($(O) + (248:2cm)$) arc (248:295:2cm)
  --
  ($(O) + (295:2.5cm)$) arc (295:248:2.5cm)
  -- cycle;
  \draw[fill=red,opacity=0.6]
  ($(O) + (305:2cm)$) arc (305:345:2cm)
  --
  ($(O) + (345:2.5cm)$) arc (345:305:2.5cm)
  -- cycle;
  \draw[fill=red,opacity=0.6]
  ($(O) + (148:2cm)$) arc (148:192:2cm)
  --
  ($(O) + (192:2.5cm)$) arc (192:148:2.5cm)
  -- cycle;
\filldraw (2.5,0)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (0.4,-0.4)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (-0.3,0.7)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (0.2,0.6)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (-0.5,-0.3)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (-0.4,0.2)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (0.7,0.5)  circle (2pt) node[anchor=north] {};
\filldraw[blue,opacity=0.7] (0,-0.7)  circle (2pt) node[anchor=north] {};
\filldraw[yellow,opacity=0.7] (0,-2.3)  circle (2pt) node[anchor=north] {};
\filldraw[yellow,opacity=0.7] (1.45,-1.55)  circle (2pt) node[anchor=north] {};
\filldraw[yellow,opacity=0.7] (-1,2.1)  circle (2pt) node[anchor=north] {};
\filldraw[yellow,opacity=0.7] (2.05,1.05)  circle (2pt) node[anchor=north] {};
\filldraw[yellow,opacity=0.7] (-2.05,0.65)  circle (2pt) node[anchor=north] {};
\draw[->,very thick, opacity=0.6] (2.3,-2.7) -- (1.5,-1.65) node[anchor=north,xshift=30pt, yshift=-30pt,opacity=1] {Adversary $a_L$};
\draw[->,very thick, opacity=0.6] (3.3,1.3) -- (2.15,1.06) node[anchor=north,xshift=40pt, yshift=20pt,opacity=1] {Adversary $a_1$};
\draw[->,very thick, opacity=0.6] (0,-1.2) -- (0,-0.8) node[anchor=north,xshift=1pt, yshift=-8pt,opacity=1] {Agent};
\draw[->,very thick, opacity=0.6] (3.2,-0.5) -- (2.6,-0.05) node[anchor=north,xshift=30pt, yshift=-9pt,opacity=1] {Client};

\end{tikzpicture}}
\caption{An illustration of the environment. A group of agents (blue) aim to securely transmit a message to a client (black) in the presence of $L$ adversaries (yellow). Both the client and the adversaries are in the far-field region. Possible directions for each adversary $a_i$, where $i$$\in$$[L]$, is described by a direction interval $I_i$. The interval $I_0$, which is of length $\delta$, defines an adversary-free region in the environment. }
\label{fig:problem}
\vspace{-3mm}
\end{figure}

==> problem_statement_conf.tex <==
\section{Problem Statement }



We consider an environment that is illustrated in Figure \ref{fig:problem}. A group of $m$ agents aim to communicate an information sequence $S^K$ with a client, i.e., intended receiver, that is located in the direction $\theta_c$$\in$$[-\pi,\pi)$. The agents map $S^K$ to a sequence $X^N$ using an encoder $f_E$ and transmit $X^N$ by using a sequence $\{({\bf{w}}_t,\Sigma_t)\}_{t=1}^N$ of beamforming vector and artificial noise pairs. The client receives a sequence $\hat{X}^N$ and maps it to the sequence $\hat{S}^K$ using a decoder $f_D$. 

There are $L$ adversaries $\{a_i $$:$$ i$$\in$$[L]\}$ in the far-field region whose objective is to infer $S^K$ by eavesdropping on the transmission of $X^N$. It is assumed that the encoder-decoder pair ($f_E,f_D$) is available at the adversaries. The exact directions of the adversaries are unknown; however, there exists a continuous interval $I_i$$\subseteq$$[-\pi,\pi)$ for each adversary $a_i$ that represents all possible directions of the adversary. Let $\mathcal{O}_i$$=$$\{t$$\in$$[N]: \text{SINR}_t(\theta)$$>$$\gamma_a\ \  \text{for some}\ \  \theta$$\in$$I_i\}$ be the set of time steps that the adversary $a_i$ observes the transmitted message bit with a nonzero probability. Then, the adversary $a_i$'s maximum information regarding $X^N$ is described by the sequence $Z^{N,i}$$=$$(Z_1^i,Z_2^i,\ldots, Z_N^i)$ which is defined in \eqref{obs_seq}.

We assume that there is an adversary-free direction interval $I_0$$=$$[\theta_c$$-$$\delta/2,\theta_c$$+$$\delta/2]$ of length $\delta$$\in$$[-\pi,\pi)$ in the environment. This assumption is necessary for the agents to communicate with the client securely because, otherwise, an adversary in the direction interval $I_0$ might receive the same signals with the client.

We are interested in to develop a transmission strategy, together with an encoding/decoding scheme, that enables the agents to communicate $S^K$ with the client while leaking no information to the adversaries. The formal problem statement is as follows.

\noindent \textbf{Problem 1: (Secure communication)} Given a client direction $\theta_c$ and a set $I_0$$\cup$$\{I_i : i$$\in$$[L]\}$ of direction intervals, design an encoder-decoder pair ($f_E,f_D$) and a sequence $\{({\bf{w}}_t^{\star}, \Sigma_t^{\star})\}_{t=1}^N$ such that $P_e$$=$$0$ and $\min_{i\in [L]}\Delta_i$$\geq$$K$$-$$\epsilon$ for any $\epsilon$$>$$0$.







